PIM-QAT: Neural Network Quantization for Processing-In-Memory (PIM) Systems

Processing-in-memory (PIM), an increasingly studied neuromorphic hardware, promises orders of energy and throughput improvements for deep learning inference. Leveraging the massively parallel and efficient analog computing inside memories, PIM circumvents the bottlenecks of data movements in conventional digital hardware. However, an extra quantization step (i.e. PIM quantization), typically with limited resolution due to hardware constraints, is required to convert the analog computing results into digital domain. Meanwhile, non-ideal effects extensively exist in PIM quantization because of the imperfect analog-to-digital interface, which further compromises the inference accuracy. In this paper, we propose a method for training quantized networks to incorporate PIM quantization, which is ubiquitous to all PIM systems. Specifically, we propose a PIM quantization aware training (PIM-QAT) algorithm, and introduce rescaling techniques during backward and forward propagation by analyzing the training dynamics to facilitate training convergence. We also propose two techniques, namely batch normalization (BN) calibration and adjusted precision training, to suppress the adverse effects of non-ideal linearity and stochastic thermal noise involved in real PIM chips. Our method is validated on three mainstream PIM decomposition schemes, and physically on a prototype chip. Comparing with directly deploying conventionally trained quantized model on PIM systems, which does not take into account this extra quantization step and thus fails, our method provides significant improvement. It also achieves comparable inference accuracy on PIM systems as that of conventionally quantized models on digital hardware, across CIFAR10 and CIFAR100 datasets using various network depths for the most popular network topology.

==> figs/fig_bn_calib_ideal_ADC.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=.8\linewidth]{imgs/bn_calib_ideal_ADC.pdf}
\caption{
\todo{}.
}
\label{fig:bn_calib_ideal_ADC_single}
\end{figure*}

==> figs/fig_bn_calib_real_ADC.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=.8\linewidth]{imgs/bn_calib_real_ADC.pdf}
\caption{
\todo{}.
}
\label{fig:bn_calib_real_ADC_single}
\end{figure*}

==> figs/fig_motivation.tex <==
\begin{figure*}[t!]
\centering
% \hspace*{-80pt}
\includegraphics[width=0.95\linewidth]{imgs/fig1.pdf}
% \includegraphics[width=0.95\linewidth]{imgs/model_explain.pdf}
\caption{
% % \textbf{Left}: Knowledge distillation with MSE loss requires extra learnable layers to map features from student ($X_s^{l}$) into the same number of channels as teacher ($X_t^(l)$). \textbf{Right}: Our proposed GCKA
% % maximizes similarity between features directly.
% \textbf{Left}: Knowledge distillation with MSE loss requires extra learnable layers to map features into the same number of channels. \textbf{Right}: Our proposed GCKA
% maximizes similarity between features directly.
% % llation technique. Unlike knowledge distillation with MSE loss, maximizing similarity between features from two models is more direct and does not require introducing extra learnable layers.
%Implementing MAC on a processing in-memory (PIM) system. (a) A PIM macro and its chip implementation. (b) Non-idealities introduced by real PIM systems, including quantization, non-linearity and noise. (c) Impact of the non-idealities on the model accuracy.
% Implementing MAC on a processing in-memory (PIM) system. (a) Principle of PIM and one real chip implementation. (b) Non-idealities introduced by real PIM systems, including quantization, non-linearity and noise (\todo{which are from hardware}). (c) Accuracy loss with conventional training and quantization. (d) Workflow of our proposed framework. (e) Performance with our proposed framework.
\textcolor{red}{\bf Very detailed caption} The problem of implementing MAC on a processing in-memory (PIM) system and our proposed solution. Compared with directly applying model trained with conventional quantization technique on PIM system, our framework significantly reduces the accuracy gap and improve the robustness agains non-idealities introduced by real PIM systems, including quantization as well as non-linearity and noise.~\zyc{explain that the reason we do not incorporate nonidealities such as imperfect linearity and thermal noise is that the chip-to-chip variation is not easy to model directly and we propose to use BN calibration to alleviate the problem}
}\label{fig:motivation}
\vskip -5ex
\end{figure*}






% \begin{figure*}[]
% \centering
% \hspace*{-80pt}
% \scalebox{1.3}{
% \begin{subfigure}[t]{.54\textwidth}
% \centering
% \includegraphics[width=\linewidth]{imgs/motivation.pdf}
% \label{fig:nonideal}
% \end{subfigure}
% % \quad
% \begin{subfigure}[t]{.12\textwidth}
% \raisebox{-0.10\linewidth}{
% \centering
% \includegraphics[width=1.8\linewidth]{imgs/baseline_problem_ps.pdf}
% % \includegraphics[width=1.2\linewidth]{imgs/baseline_problem.pdf}
% \label{fig:baseline_problem}
% }
% \end{subfigure}
% }
% \caption{
% % % \textbf{Left}: Knowledge distillation with MSE loss requires extra learnable layers to map features from student ($X_s^{l}$) into the same number of channels as teacher ($X_t^(l)$). \textbf{Right}: Our proposed GCKA
% % % maximizes similarity between features directly.
% % \textbf{Left}: Knowledge distillation with MSE loss requires extra learnable layers to map features into the same number of channels. \textbf{Right}: Our proposed GCKA
% % maximizes similarity between features directly.
% % % llation technique. Unlike knowledge distillation with MSE loss, maximizing similarity between features from two models is more direct and does not require introducing extra learnable layers.
% Implementing MAC on a processing in-memory (PIM) system. Left: A PIM macro and its chip implementation. Middle: Non-idealities introduced by real PIM systems, including quantization, non-linearity and noise. Right: Impact of the non-idealities on the model accuracy.
% }\label{fig:motivation}
% \end{figure*}



% \begin{figure*}[h]
% \centering
% \includegraphics[width=.8\linewidth]{imgs/motivation.pdf}
% \caption{
% \todo{Motivation}.
% }
% \label{fig:noise}
% \end{figure*}

==> figs/fig_noise_6bit_ideal_ADC.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=.8\linewidth]{imgs/noise_6bit_ideal_ADC.pdf}
\caption{
\todo{}.
}
\label{fig:noise_6bit_ideal}
\end{figure*}

==> figs/fig_noise_7bit_ideal_ADC.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=.8\linewidth]{imgs/noise_7bit_ideal_ADC.pdf}
\caption{
\todo{}.
}
\label{fig:noise_7bit_ideal}
\end{figure*}

==> figs/fig_noise_7bit_real_ADC.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=.8\linewidth]{imgs/noise_7bit_real_ADC.pdf}
\caption{
\todo{}.
}
\label{fig:noise_7bit_real}
\end{figure*}

==> figs/fig_noise_8bit_ideal_ADC.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=.8\linewidth]{imgs/noise_8bit_ideal_ADC.pdf}
\caption{
\todo{}.
}
\label{fig:noise_8bit_ideal}
\end{figure*}

==> figs/fig_statistics.tex <==
\begin{figure}[h]
\centering
\hskip -4.5ex
\begin{subfigure}[t]{.8\linewidth}
\centering
\includegraphics[width=\linewidth]{imgs/bit_adc_std_ratio_sigma_0.pdf}
\vskip -2ex
\caption{}
\label{fig:std_ratio}
\vskip -4.5ex
\end{subfigure}
%\hskip -4ex
\vskip -.5ex
\begin{subfigure}[t]{\linewidth}
% \raisebox{0.008\linewidth}{
\centering
\includegraphics[width=\linewidth]{imgs/running_stats_nonideality.pdf}
% }
\vskip -2ex
\caption{}
\label{fig:running_stats_nonideality}
\vskip -4.5ex
\end{subfigure}
\vskip -2ex
\caption{Running statistics changing caused by non-ideal effects.
(a) Impact of PIM-quantization on the output running statistics. (b) Impact of non-linearity and noise on the output running statistics. Note this is one sampling results.
}
\label{fig:running_stats}
\end{figure}




==> figs/fig_workflow.tex <==
% \vskip -2ex
\begin{figure}[!t]
\centering
\includegraphics[width=.75\linewidth]{imgs/workflow.pdf}
% \vskip -2ex
\caption{
Workflow of our general framework.
}
\label{fig:workflow}
% \vskip -3ex
\end{figure}

==> tabs/tab_adjusted_bit_training.tex <==
\begin{table*}[t]
\caption{\todo{Adjusted Bit Training with CIFAR10}.}
\label{tab:adjust_bit_training}
% \vskip 0.15in
\vspace{-15pt}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cccccccc}
\toprule
\multirow{2}{*}{Method} & ADC & \multirow{2}{*}{ADC Type} & \multirow{2}{*}{Noise Level} & \multirow{2}{*}{ENOB} & Training ADC & Top-1 & Top-5 \\
& Resolution &&&& Resolution & Acc. & Acc. \\
\midrule
\multirow{12}{*}{Baseline} & \multirow{12}{*}{7} & \multirow{12}{*}{Real} & \multirow{3}{*}{0.0} & \multirow{3}{*}{6.13} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\cmidrule{4-8}
&  &  & \multirow{3}{*}{0.2} & \multirow{3}{*}{5.37} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\cmidrule{4-8}
&  &  & \multirow{3}{*}{0.35} & \multirow{3}{*}{4.98} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\cmidrule{4-8}
&  &  & \multirow{3}{*}{0.5} & \multirow{3}{*}{4.68} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\midrule
\multirow{12}{*}{AMS} & \multirow{12}{*}{7} & \multirow{12}{*}{Real} & \multirow{3}{*}{0.0} & \multirow{3}{*}{6.13} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\cmidrule{4-8}
&  &  & \multirow{3}{*}{0.2} & \multirow{3}{*}{5.37} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\cmidrule{4-8}
&  &  & \multirow{3}{*}{0.35} & \multirow{3}{*}{4.98} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\cmidrule{4-8}
&  &  & \multirow{3}{*}{0.5} & \multirow{3}{*}{4.68} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\midrule
\multirow{12}{*}{Ours} & \multirow{12}{*}{7} & \multirow{12}{*}{Real} & \multirow{3}{*}{0.0} & \multirow{3}{*}{6.13} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\cmidrule{4-8}
&  &  & \multirow{3}{*}{0.2} & \multirow{3}{*}{5.37} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\cmidrule{4-8}
&  &  & \multirow{3}{*}{0.35} & \multirow{3}{*}{4.98} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\cmidrule{4-8}
&  &  & \multirow{3}{*}{0.5} & \multirow{3}{*}{4.68} & 7 &  & \\
&  &  &  &  & 6 &  & \\
&  &  &  &  & 5 &  & \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\end{table*}

==> tabs/tab_bn_calib.tex <==
\begin{table*}[t]
\caption{\todo{BN Calibration with CIFAR10 (ideal \& real ADC)} (wo adjusted bit training).}
\label{tab:bn_calib}
% \vskip 0.15in
\vspace{-15pt}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{ADC Type} & \multirow{2}{*}{Noise Level} & \multicolumn{2}{c}{Top-1 Acc.} & \multicolumn{2}{c}{Top-5 Acc.} \\
&&& w/o BN & w/ BN & w/o BN & w/ BN \\
\midrule
\multirow{8.5}{*}{Baseline} & \multirow{4}{*}{Ideal} & 0.0 & 85.8 & 87.3 & 98.9 & 99.2 \\
& & 0.2 & 79.2 & 82.6 & 96.6 & 98.6 \\
& & 0.35 & 62.3 & 71.2 & 87.8 & 96.0 \\
& & 0.5 & 35.6 & 48.6 & 77.7 & 88.1 \\
\cmidrule{2-7}
& \multirow{4}{*}{Real} & 0.0 & 12.1 & 56.5 & 58.5 & 91.0 \\
& & 0.2 & 11.5 & 51.9 & 58.1 & 89.3 \\
& & 0.35 & 10.9 & 40.7 & 57.8 & 84.9 \\
& & 0.5 & 10.8 & 28.9 & 58.5 & 77.5 \\
\midrule
% \multirow{6.5}{*}{AMS}  & \multirow{3}{*}{N} & 0.2 & 83.7 & 99.4 \\
% & & 0.35 & 82.9 & 99.3 \\
% & & 0.5 & 81.2 & 99.2 \\
% \cmidrule{2-7}
% & \multirow{3}{*}{Y} & 0.2 & 88.0 & 99.6 \\
% & & 0.35 & 87.7 & 99.6 \\
% & & 0.5 & 86.9 & 99.5 \\
% \midrule
\multirow{8.5}{*}{Ours} & \multirow{4}{*}{Ideal} & 0.0 & 90.1 & 90.2 & 99.5 & 99.6 \\
& & 0.2 & 89.4 & 89.7 & 99.6 & 99.7 \\
& & 0.35 & 88.8 & 88.8 & 99.5 & 99.6 \\
& & 0.5 & 86.0 & 87.0 & 99.2 & 99.5 \\
\cmidrule{2-7}
& \multirow{4}{*}{Real} & 0.0 & 58.7 & 86.6 & 93.2 & 99.3 \\
& & 0.2 & 58.5 & 86.2 & 92.9 & 99.4 \\
& & 0.35 & 57.0 & 84.8 & 92.1 & 99.3 \\
& & 0.5 & 53.9 & 82.1 & 90.2 & 99.3 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\end{table*}






















% \begin{table*}[t]
% \caption{\todo{BN Calibration with CIFAR10 (ideal \& real ADC)} (wo adjusted bit training).}
% \label{tab:bn_calib}
% % \vskip 0.15in
% \vspace{-15pt}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{ccccccc}
% \toprule
% \multirow{2}{*}{Method} & \multirow{2}{*}{BN Calib.} & \multirow{2}{*}{Noise Level} & \multicolumn{2}{c}{Top-1 Acc.} & \multicolumn{2}{c}{Top-5 Acc.} \\
% &&& Ideal ADC & Real ADC & Ideal ADC & Real ADC \\
% \midrule
% \multirow{8.5}{*}{Baseline} & \multirow{4}{*}{N} & 0.0 & 85.8 & 12.1 & 98.9 & 58.5 \\
% & & 0.2 & 79.2 & 11.5 & 96.6 & 58.1 \\
% & & 0.35 & 62.3 & 10.9 & 87.8 & 57.8 \\
% & & 0.5 & 35.6 & 10.8 & 77.7 & 58.5 \\
% \cmidrule{2-7}
% & \multirow{4}{*}{Y} & 0.0 & 87.3 & 56.5 & 99.2 & 91.0 \\
% & & 0.2 & 82.6 & 51.9 & 98.6 & 89.3 \\
% & & 0.35 & 71.2 & 40.7 & 96.0 & 84.9 \\
% & & 0.5 & 48.6 & 28.9 & 88.1 & 77.5 \\
% \midrule
% % \multirow{6.5}{*}{AMS}  & \multirow{3}{*}{N} & 0.2 & 83.7 & 99.4 \\
% % & & 0.35 & 82.9 & 99.3 \\
% % & & 0.5 & 81.2 & 99.2 \\
% % \cmidrule{2-7}
% % & \multirow{3}{*}{Y} & 0.2 & 88.0 & 99.6 \\
% % & & 0.35 & 87.7 & 99.6 \\
% % & & 0.5 & 86.9 & 99.5 \\
% % \midrule
% \multirow{8.5}{*}{Ours} & \multirow{4}{*}{N} & 0.0 & 90.1 & 58.7 & 99.5 & 93.2 \\
% & & 0.2 & 89.4 & 58.5 & 99.6 & 92.9 \\
% & & 0.35 & 88.8 & 57.0 & 99.5 & 92.1 \\
% & & 0.5 & 86.0 & 53.9 & 99.2 & 90.2 \\
% \cmidrule{2-7}
% & \multirow{4}{*}{Y} & 0.0 & 90.2 & 86.6 & 99.6 & 99.3 \\
% & & 0.2 & 89.7 & 86.2 & 99.7 & 99.4 \\
% & & 0.35 & 88.8 & 84.8 & 99.6 & 99.3 \\
% & & 0.5 & 87.0 & 82.1 & 99.5 & 99.3 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% % \vskip -0.1in
% \end{table*}



















% \begin{table*}[t]
% \caption{\todo{BN Calibration with CIFAR10 (real ADC)} (wo adjusted bit training).}
% \label{tab:bn_calib}
% % \vskip 0.15in
% \vspace{-15pt}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{ccccc}
% \toprule
% Method & BN Calib. & Noise Level & Top-1 Acc. & Top-5 Acc. \\
% \midrule
% \multirow{8.5}{*}{Baseline}  & \multirow{4}{*}{N} & 0.0 & 12.1 & 58.5 \\
% & & 0.2 & 11.5 & 58.1 \\
% & & 0.35 & 10.9 & 57.8 \\
% & & 0.5 & 10.8 & 58.5 \\
% \cmidrule{2-5}
% & \multirow{4}{*}{Y} & 0.0 & 56.5 & 91.0 \\
% & & 0.2 & 51.9 & 89.3 \\
% & & 0.35 & 40.7 & 84.9 \\
% & & 0.5 & 28.9 & 77.5 \\
% \midrule
% % \multirow{6.5}{*}{AMS}  & \multirow{3}{*}{N} & 0.2 & 83.7 & 99.4 \\
% % & & 0.35 & 82.9 & 99.3 \\
% % & & 0.5 & 81.2 & 99.2 \\
% % \cmidrule{2-5}
% % & \multirow{3}{*}{Y} & 0.2 & 88.0 & 99.6 \\
% % & & 0.35 & 87.7 & 99.6 \\
% % & & 0.5 & 86.9 & 99.5 \\
% % \midrule
% \multirow{8.5}{*}{Ours}  & \multirow{4}{*}{N} & 0.0 & 58.7 & 93.2 \\
% & & 0.2 & 58.5 & 92.9 \\
% & & 0.35 & 57.0 & 92.1 \\
% & & 0.5 & 53.9 & 90.2 \\
% \cmidrule{2-5}
% & \multirow{4}{*}{Y} & 0.0 & 86.6 & 99.3 \\
% & & 0.2 & 86.2 & 99.4 \\
% & & 0.35 & 84.8 & 99.3 \\
% & & 0.5 & 82.1 & 99.3 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% % \vskip -0.1in
% \end{table*}


% \begin{table*}[t]
% \caption{\todo{BN Calibration with CIFAR10 (ideal ADC)} (wo adjusted bit training).}
% \label{bn_calib_ideal_adc}
% % \vskip 0.15in
% \vspace{-15pt}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{ccccc}
% \toprule
% Method & BN Calib. & Noise Level & Top-1 Acc. & Top-5 Acc. \\
% \midrule
% \multirow{8.5}{*}{Baseline}  & \multirow{4}{*}{N} & 0.0 & 85.8 & 98.9 \\
% & & 0.2 & 79.2 & 96.6 \\
% & & 0.35 & 62.3 & 87.8 \\
% & & 0.5 & 35.6 & 77.7 \\
% \cmidrule{2-5}
% & \multirow{4}{*}{Y} & 0.0 & 87.3 & 99.2 \\
% & & 0.2 & 82.6 & 98.6 \\
% & & 0.35 & 71.2 & 96.0 \\
% & & 0.5 & 48.6 & 88.1 \\
% \midrule
% % \multirow{6.5}{*}{AMS}  & \multirow{3}{*}{N} & 0.2 & 89.5 & 99.6 \\
% % & & 0.35 & 89.0 & 99.6 \\
% % & & 0.5 & 88.6 & 99.5 \\
% % \cmidrule{2-5}
% % & \multirow{3}{*}{Y} & 0.2 & 89.6 & 99.5 \\
% % & & 0.35 & 89.2 & 99.6 \\
% % & & 0.5 & 88.9 & 99.5 \\
% % \midrule
% \multirow{8.5}{*}{Ours}  & \multirow{4}{*}{N} & 0.0 & 90.1 & 99.5 \\
% & & 0.2 & 89.4 & 99.6 \\
% & & 0.35 & 88.8 & 99.5 \\
% & & 0.5 & 86.0 & 99.2 \\
% \cmidrule{2-5}
% & \multirow{4}{*}{Y} & 0.0 & 90.2 & 99.6 \\
% & & 0.2 & 89.7 & 99.7 \\
% & & 0.35 & 88.8 & 99.6 \\
% & & 0.5 & 87.0 & 99.5 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% % \vskip -0.1in
% \end{table*}

==> tabs/tab_cifar100_comp.tex <==
\begin{table}[t]
\caption{\todo{CIFAR100 comparison with 7bit real ADC of 0.35 noise level}.}%(Best result for each method?)}.}
\label{tab:cifar100}
% \vskip 0.15in
\vspace{-15pt}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{ccc}
\toprule
Method & Top-1 Acc. & Top-5 Acc. \\
\midrule
Baseline & 1.6 & 7.3 \\
AMS & 44.9 & 77.3 \\
Ours (wo/ BN calib.) & 50.7 & 80.2 \\
\textbf{Ours (w/ BN calib.)} & \textbf{61.5} & \textbf{87.6} \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\end{table}










% \begin{table}[t]
% \caption{\todo{CIFAR100 comparison with 7bit real ADC of 0.35 noise level}.}%(Best result for each method?)}.}
% \label{cifar100_comp}
% % \vskip 0.15in
% \vspace{-15pt}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{ccc}
% \toprule
% Method & Top-1 Acc. & Top-5 Acc. \\
% \midrule
% Baseline & 1.6 & 7.3 \\
% AMS & 44.9 & 77.3 \\
% Ours (wo/ BN calib.) & 50.7 & 80.2 \\
% \textbf{Ours (w/ BN calib.)} & \textbf{61.5} & \textbf{87.6} \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% % \vskip -0.1in
% \end{table}






% \begin{table*}[t]
% \caption{\todo{CIFAR100 Comparison (Best result for each method?)}.}
% \label{cifar100_comp}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{ccccc}
% \toprule
% Method & ENOB & Noise Level & Top-1 Acc. & Top-5 Acc. \\
% \midrule
% Baseline   & 6.13 & 0.35 & 11.6 & 33.9 \\
% AMS & 6.13 & 0.35 & 60.4 & 86.9 \\
% Ours & 6.13 & 0.35 & 61.3 & 87.4 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}

==> tabs/tab_cifar10_comp.tex <==
\begin{table}[t]
\caption{\todo{ResNet results with 7bit processing in-memory system of noise level 0.35}.}%(Best result for each method?)}.}
\label{tab:cifar10}
% \vskip 0.15in
\vspace{-15pt}
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cccc}
\toprule
Dataset & Depth & Top-1 Acc. & Top-5 Acc. \\
\midrule
\multirow{4}{*}{CIFAR10} & 20 & 89.1 & 99.6 \\
& 32 & 89.3 & 99.7 \\
& 44 & 90.7 & 99.7 \\
& 56 & 90.4 & 99.7 \\
\midrule
CIFAR100 & 20 & 61.8 & 87.5 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
% \vskip -0.1in
\end{table}
















% \begin{table}[t]
% \caption{\todo{CIFAR10 comparison with 7bit real ADC of 0.35 noise level}.}%(Best result for each method?)}.}
% \label{cifar10_comp}
% % \vskip 0.15in
% \vspace{-15pt}
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{ccc}
% \toprule
% Method & Top-1 Acc. & Top-5 Acc. \\
% \midrule
% Baseline   & 11.2 & 57.9 \\
% AMS & 83.1 & 99.3 \\
% Ours (wo/ BN calib.) & 84.1 & 99.3 \\
% \textbf{Ours (w/ BN calib.)} & \textbf{88.7} & \textbf{99.7} \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% % \vskip -0.1in
% \end{table}







% \begin{table*}[t]
% \caption{\todo{CIFAR10 Comparison (Best result for each method?)}.}
% \label{cifar10_comp}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{ccccc}
% \toprule
% Method & ENOB & Noise Level & Top-1 Acc. & Top-5 Acc. \\
% \midrule
% Baseline   & 6.13 & 0.35 & 41.0 & 84.9 \\
% AMS & 6.13 & 0.35 & 88.1 & 99.6 \\
% Ours & 6.13 & 0.35 & 89.0 & 99.6 \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}

==> tabs/tab_result_comp.tex <==
\begin{table*}[ht]
\scalebox{.9}{
\begin{minipage}[b]{0.5\linewidth}
\centering
\includegraphics[width=\linewidth]{imgs/result_comp_N72.pdf}\\
\includegraphics[width=\linewidth]{imgs/result_comp_N72.pdf}
\captionof{figure}{2-D scatterplot of the Student Database}
\label{fig:res_comp_fig}
\end{minipage}
\hspace{2pt}
\begin{minipage}[b]{0.32\linewidth}
\centering
\begin{tabular}{cccccc}
\toprule
Dataset & Depth & Method & N & Top-1 Acc. & Top-5 Acc. \\
\midrule
\multirow{21.5}{*}{CIFAR10} & \multirow{5}{*}{20} & Software & - & 91.6 & 99.7 \\
& & \multirow{2}{*}{Baseline} & 72 & 13.9 & 57.5 \\
& & & 144 & 10.9 & 57.8 \\
& & \multirow{2}{*}{Ours} & 72 & 89.7 & 99.7 \\
& & & 144 & 89.1 & 99.6 \\
\cmidrule{2-6}
& \multirow{5}{*}{32} & Software & - & 92.5 & 99.6 \\
& & \multirow{2}{*}{Baseline} & 72 & 10.0 & 52.0 \\
& & & 144 & 10.1 & 50.0 \\
& & \multirow{2}{*}{Ours} & 72 & 90.6 & 99.6 \\
& & & 144 & 89.3 & 99.7 \\
\cmidrule{2-6}
& \multirow{5}{*}{44} & Software & - & 92.8 & 99.7 \\
& & \multirow{2}{*}{Baseline} & 72 & 10.5 & 50.1 \\
& & & 144 & 10.0 & 50.1 \\
& & \multirow{2}{*}{Ours} & 72 & 90.6 & 99.7 \\
& & & 144 & 90.7 & 99.7 \\
\cmidrule{2-6}
& \multirow{5}{*}{56} & Software & - & 92.4 & 99.7 \\
& & \multirow{2}{*}{Baseline} & 72 & 10.0 & 50.0 \\
& & & 144 & 10.0 & 50.0 \\
& & \multirow{2}{*}{Ours} & 72 & 90.7 & 99.7 \\
& & & 144 & 90.4 & 99.7 \\
\midrule
\multirow{5}{*}{CIFAR100} & \multirow{5}{*}{20} & Software & - & 67.0 & 89.6 \\
& & \multirow{2}{*}{Baseline} & 72 & 1.3 & 6.2 \\
& & & 144 & 1.8 & 8.6 \\
& & \multirow{2}{*}{Ours} & 72 & 62.6 & 88.2 \\
& & & 144 & 61.8 & 87.5 \\
\bottomrule
\end{tabular}
\caption{Student Database}
\label{table:student}
\end{minipage}\hfill
}
\end{table*}

==> tex_files/A1_proof_one_column.tex <==
\section{Proof of Theorems}
\label{sec:proof}

Here we present detailed proofs for Theorem 1 and 2. We first formulate the quantization procedure of PIM systems with several popular schemes, then derive the results of Theorem 1. After that, we analyze the training dynamics of a generic neural networks to prove Theorem 2.

\subsection{PIM Quantization-Aware Training}
To prove Theorem 1, we first present the quantization procedure of PIM systems with native, differential and bit serial schemes. The output of a linear layer is given by
\begin{equation}
    \widetilde{y}=\sum_{i=1}^N\widetilde{Q}_i\widetilde{q}_i
\end{equation}
where $\widetilde{Q}_i\in[-1,1]$ is quantized weight of $b_w$ bits and $\widetilde{q}_i\in[0,1]$ is quantized input of $b_a$ bits, respectively.

For PIM systems, due to the limited resolution of digital-to-analog converter (which is $m$ bits) for the inputs, the inputs are first decomposed into sub-arrays of $m$ bits. In other words, we have
\begin{subequations}
\allowdisplaybreaks
\begin{align}
    \widetilde{q}_i&=\sum_{k=0}^{b_a/m-1}\widetilde{q}^{(m)}_{i,k}\Delta^k\\
    \widetilde{q}^{(m)}_{i,k}&=\frac{1}{2^{b_a}-1}q^{(m)}_{i,k}\\
    \Delta&=2^m
\end{align}
\end{subequations}
with $q^{(m)}_{i,k}\in\{0,1,\dots,\Delta-1\}$.%, and its derivative is given as
% \begin{equation}
%     \mathrm{d}\widetilde{q}_i=\sum_{k=0}^{b_a/m-1}\Delta^k\mathrm{d}\widetilde{q}^{(m)}_{i,k}
% \end{equation}

\paragraph{Native Scheme} For PIM system with native scheme, the output is given by
\begin{subequations}
\allowdisplaybreaks
\begin{align}
    \widetilde{y}_{\IMC}&=\bm{\mathsf{Q}}\bigg(\sum_{i=1}^N\widetilde{Q}_i\widetilde{q}_i;b_{\IMC}\bigg)\\
    &=\sum_{k=0}^{b_a/m-1}\Delta^k\cdot\frac{N(\Delta-1)}{(2^{b_{\IMC}}-1)(2^{b_a}-1)}\cdot\round\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N\widetilde{Q}_i\cdot \widetilde{q}^{(m)}_{i,k}\Big)\label{eq:native}
\end{align}
\end{subequations}
With the GSTE assumption, we can derive its differential as
\begin{subequations}
\allowdisplaybreaks
\begin{align}
    \mathrm{d}\widetilde{y}_{\IMC}&=\sum_{k=0}^{b_a/m-1}\Delta^k\cdot\frac{N(\Delta-1)}{(2^{b_{\IMC}}-1)(2^{b_a}-1)}\cdot\mathrm{d}\Big[\round\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N\widetilde{Q}_i\cdot \widetilde{q}^{(m)}_{i,k}\Big)\Big]\\
    &=\sum_{k=0}^{b_a/m-1}\Delta^k\cdot\frac{N(\Delta-1)}{(2^{b_{\IMC}}-1)(2^{b_a}-1)}\cdot\xi\cdot\mathrm{d}\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N\widetilde{Q}_i\cdot \widetilde{q}^{(m)}_{i,k}\Big)\\
    &=\xi\cdot\mathrm{d}\Big(\sum_{i=1}^N\widetilde{Q}_i\cdot \sum_{k=0}^{b_a/m-1}\widetilde{q}^{(m)}_{i,k}\Delta^k\Big)\\
    &=\xi\cdot\mathrm{d}\bigg(\sum_{i=1}^N\widetilde{Q}_i\widetilde{q}_i\bigg)\label{eq:native_diff}
\end{align}
\end{subequations}

\paragraph{Differential Scheme} For PIM system with differential scheme, the weight is first decomposed into positive and negative parts, as
\begin{equation}
    \widetilde{Q}_i=\widetilde{Q}_i^+ +\widetilde{Q}_i^-
\end{equation}
where all elements in $\widetilde{Q}_i^+$ are positive and those in $\widetilde{Q}_i^-$ are negative. Its differential is given by
\begin{equation}
    \mathrm{d}\widetilde{Q}_i=\mathrm{d}\widetilde{Q}_i^+ +\mathrm{d}\widetilde{Q}_i^-
\end{equation}
The output is the combination of these two parts as
\begin{subequations}
\allowdisplaybreaks
\begin{align}
    \widetilde{y}_{\IMC}&=\bm{\mathsf{Q}}\bigg(\sum_{i=1}^N\widetilde{Q}_i\widetilde{q}_i;b_{\IMC}\bigg)\\
    &=\sum_{k=0}^{b_a/m-1}\Delta^k\cdot\frac{N(\Delta-1)}{(2^{b_{\IMC}}-1)(2^{b_a}-1)}\cdot\Big[\round\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N\widetilde{Q}_i^+\widetilde{q}^{(m)}_{i,k}\Big)\nonumber\\
    &\quad-\round\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N(-\widetilde{Q}_i^-)\widetilde{q}^{(m)}_{i,k}\Big)\Big]\label{eq:differential}
\end{align}
\end{subequations}
Taking differential on both sides gives
\begin{subequations}
\allowdisplaybreaks
\begin{align}
    \mathrm{d}\widetilde{y}_{\IMC}&=\mathrm{d}\sum_{k=0}^{b_a/m-1}\Delta^k\cdot\frac{N(\Delta-1)}{(2^{b_{\IMC}}-1)(2^{b_a}-1)}\cdot\Big[\round\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N\widetilde{Q}_i^+\widetilde{q}^{(m)}_{i,k}\Big)\nonumber\\
    &\quad-\round\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N(-\widetilde{Q}_i^-)\widetilde{q}^{(m)}_{i,k}\Big)\Big]\\
    &=\sum_{k=0}^{b_a/m-1}\Delta^k\cdot\frac{N(\Delta-1)}{(2^{b_{\IMC}}-1)(2^{b_a}-1)}\cdot\Big\{\mathrm{d}\Big[\round\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N\widetilde{Q}_i^+\widetilde{q}^{(m)}_{i,k}\Big)\Big]\nonumber\\
    &\quad-\mathrm{d}\Big[\round\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N(-\widetilde{Q}_i^-)\widetilde{q}^{(m)}_{i,k}\Big)\Big]\Big\}\\
    &=\sum_{k=0}^{b_a/m-1}\Delta^k\cdot\frac{N(\Delta-1)}{(2^{b_{\IMC}}-1)(2^{b_a}-1)}\cdot\Big[\xi\cdot\mathrm{d}\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N\widetilde{Q}_i^+\widetilde{q}^{(m)}_{i,k}\Big)\nonumber\\
    &\quad-\xi\cdot\mathrm{d}\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N(-\widetilde{Q}_i^-)\widetilde{q}^{(m)}_{i,k}\Big)\Big]\\
    &=\xi\cdot\mathrm{d}\Big(\sum_{i=1}^N\widetilde{Q}_i^+\sum_{k=0}^{b_a/m-1}\widetilde{q}^{(m)}_{i,k}\Delta^k\Big)+\xi\cdot\mathrm{d}\Big(\sum_{i=1}^N\widetilde{Q}_i^-\sum_{k=0}^{b_a/m-1}\widetilde{q}^{(m)}_{i,k}\Delta^k\Big)\\
    &=\xi\cdot\mathrm{d}\Big(\sum_{i=1}^N\widetilde{Q}_i^+\widetilde{q}_i\Big)+\xi\cdot\mathrm{d}\Big(\sum_{i=1}^N\widetilde{Q}_i^-\widetilde{q}_i\Big)\\
    &=\xi\cdot\mathrm{d}\Big(\sum_{i=1}^N(\widetilde{Q}_i^++\widetilde{Q}_i^-)\widetilde{q}_i\Big)\\
    &=\xi\cdot\mathrm{d}\bigg(\sum_{i=1}^N\widetilde{Q}_i\widetilde{q}_i\bigg)\label{eq:differential_diff}
\end{align}
\end{subequations}

\paragraph{Bit Serial Scheme} For PIM system with bit serial scheme, the weight is first decomposed into bits as
\begin{equation}
    \widetilde{Q}_i=\sum_{k=0}^{b_w-1}(-1)^{\delta_{k,b_w-1}}\widetilde{Q}_{i,k}2^k
\end{equation}
where
\begin{equation}
    \widetilde{Q}_{i,k}=\frac{1}{2^{b_w-1}-1}Q_{i,k}
\end{equation}
and $Q_{i,k}\in\{0,1\}$.
The output is obtained for each bits separately and then summed over as
\begin{subequations}
\allowdisplaybreaks
\begin{align}
    \widetilde{y}_{\IMC}&=\bm{\mathsf{Q}}\bigg(\sum_{i=1}^N\widetilde{Q}_i\widetilde{q}_i;b_{\IMC}\bigg)\\
    &=\sum_{k=0}^{b_w-1}\sum_{l=0}^{b_a/m-1}(-1)^{\delta_{k,b_w-1}}2^k\Delta^l\cdot\frac{N(\Delta-1)}{(2^{b_{\IMC}}-1)(2^{b_w-1}-1)(2^{b_a}-1)}\nonumber\\
    &\quad\cdot\round\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_w-1}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N\widetilde{Q}_{i,k}\widetilde{q}^{(m)}_{i,l}\Big)\label{eq:bit_serial}
\end{align}
\end{subequations}
The differential can thus be determined as
\begin{subequations}
\allowdisplaybreaks
\begin{align}
    \mathrm{d}\widetilde{y}_{\IMC}&=\mathrm{d}\sum_{k=0}^{b_w-1}\sum_{l=0}^{b_a/m-1}(-1)^{\delta_{k,b_w-1}}2^k\Delta^l\cdot\frac{N(\Delta-1)}{(2^{b_{\IMC}}-1)(2^{b_w-1}-1)(2^{b_a}-1)}\nonumber\\
    &\quad\cdot\round\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_w-1}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N\widetilde{Q}_{i,k}\widetilde{q}^{(m)}_{i,l}\Big)\\
    &=\sum_{k=0}^{b_w-1}\sum_{l=0}^{b_a/m-1}(-1)^{\delta_{k,b_w-1}}2^k\Delta^l\cdot\frac{N(\Delta-1)}{(2^{b_{\IMC}}-1)(2^{b_w-1}-1)(2^{b_a}-1)}\nonumber\\
    &\quad\cdot\mathrm{d}\Big[\round\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_w-1}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N\widetilde{Q}_{i,k}\widetilde{q}^{(m)}_{i,l}\Big)\Big]\\
    &=\sum_{k=0}^{b_w-1}\sum_{l=0}^{b_a/m-1}(-1)^{\delta_{k,b_w-1}}2^k\Delta^l\cdot\frac{N(\Delta-1)}{(2^{b_{\IMC}}-1)(2^{b_w-1}-1)(2^{b_a}-1)}\nonumber\\
    &\quad\cdot\xi\cdot\mathrm{d}\Big(\frac{(2^{b_{\IMC}}-1)(2^{b_w-1}-1)(2^{b_a}-1)}{N(\Delta-1)}\sum_{i=1}^N\widetilde{Q}_{i,k}\widetilde{q}^{(m)}_{i,l}\Big)\\
    &=\xi\cdot\mathrm{d}\Big(\sum_{i=1}^N\sum_{k=0}^{b_w-1}(-1)^{\delta_{k,b_w-1}}\widetilde{Q}_{i,k}2^k\cdot\sum_{l=0}^{b_a/m-1}\widetilde{q}^{(m)}_{i,l}\Delta^l\Big)\\
    &=\xi\cdot\mathrm{d}\bigg(\sum_{i=1}^N\widetilde{Q}_i\widetilde{q}_i\bigg)\label{eq:bit_serial_diff}
\end{align}
\end{subequations}

With~\eqref{eq:native_diff},~\eqref{eq:differential_diff} and~\eqref{eq:bit_serial_diff}, we prove Theorem 1.


\subsection{Training Dynamics}

Here we analyze the training dynamics to prove Theorem 2. Our analysis is similar to that presented in~\citep{quantefficienttraining}, which is zeroth order approximation and is based on mean field theory, where different quantities are assumed to be independent (although some of them have some dependence, especially the gradients, as described following Axiom 3.2 in~\citep{yang2017mean}).

We want to analyze the training dynamics of a generic neural network with repeated blocks composed of linear layer, some nonlinear effect, forward scaling, batch normalization, and output activation function, as
\begin{subequations}
\allowdisplaybreaks
\begin{align}
    x^{(l+1)}_i &= \varphi(y^{(l)}_i)\\
    y^{(l)}_i &= \gamma^{(l)}_i\frac{z^{(l)}_i-\mu^{(l)}_i}{\sigma^{(l)}_i} + \beta^{(l)}_i\\
    z^{(l)}_i &=\eta^{(l)}\widetilde{z}^{(l)}_i\\
    \widetilde{z}^{(l)}_i &= f(W^{(l)}_{ij},x^{(l)}_j)\\
    &\sim\rho^{(l)}\sum_{j=1}^{n^{(l)}}W^{(l)}_{ij}x^{(l)}_j\\
    \mathrm{d}\widetilde{z}^{(l)}_i &=\xi^{(l)}\cdot\mathrm{d}\left(\sum_{j=1}^{n^{(l)}}W^{(l)}_{ij}x^{(l)}_j\right)
\end{align}
\end{subequations}
where $\rho^{(l)}$ denotes modification on the output variance by the nonlinear effect and $\xi^{(l)}$ is the scaling factor introduced during backward propagation. From this we can derive the following statistics

\begin{subequations}
\allowdisplaybreaks
\begin{align}
    \VAR{y^{(l)}_i}&\approx(\gamma^{(l)}_i)^2\\
    \E{(x^{(l)}_i)^2}&\approx\E{(\varphi'(y^{(l)}_i))^2}\VAR{y^{(l)}_i}\label{eq:mse}\\
    &\approx\E{(\varphi'(y^{(l)}_i))^2}(\gamma^{(l)}_i)^2\\
    (\sigma^{(l)}_i)^2&=\VAR{z^{(l)}_i}\\
    &=(\eta^{(l)})^2(\rho^{(l)})^2n^{(l)}\VAR{W^{(l)}_{ij}}\E{(x^{(l)}_j)^2}\\
    &\approx (\eta^{(l)})^2(\rho^{(l)})^2n^{(l)}\VAR{W^{(l)}_{ij}}\E{(\varphi'(y^{(l)}_j))^2}(\gamma^{(l)}_j)^2\label{eq:sigma}
\end{align}
\end{subequations}
where~\eqref{eq:mse} is valid if the activation $\phi$ is quasi-linear.

We first estimate the gradient of the batch normalization layer as following
\begin{subequations}
\allowdisplaybreaks
\begin{align}
    \frac{\partial\mu^{(l)}_i}{\partial z^{(l)}_i}&=\frac{1}{m_B}\\
    \frac{\partial\sigma^{(l)}_i}{\partial z^{(l)}_i}&=\frac{1}{m_B}\frac{z^{(l)}_i-\mu^{(l)}_i}{\sigma^{(l)}_i}\\
    \frac{\partial y^{(l)}_i}{\partial z^{(l)}_i}&=\gamma^{(l)}_i\left[\frac{1}{\sigma^{(l)}_i}-\frac{1}{\sigma^{(l)}_i}\frac{\partial\mu^{(l)}_i}{\partial z^{(l)}_i}+(z^{(l)}_i-\mu^{(l)}_i)\frac{-1}{(\sigma^{(l)}_i)^2}\frac{\partial\sigma^{(l)}_i}{\partial z^{(l)}_i}\right]\\
    &=\gamma^{(l)}_i\left[\frac{1}{\sigma^{(l)}_i}-\frac{1}{\sigma^{(l)}_i}\frac{1}{m_B}-\frac{1}{\sigma^{(l)}_i}\frac{1}{m_B}\left(\frac{z^{(l)}_i-\mu^{(l)}_i}{\sigma^{(l)}_i}\right)^2\right]\\
    &\approx\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\quad(m_B>>1)
\end{align}
\end{subequations}
where we have assumed that the batch size is large enough, which is typically satisfied in practice.

The gradients of loss $L$ with respect to the input can be easily calculated, which is
\begin{equation}
    \partial_{x^{(l)}_j}L=\xi^{(l)}\sum_{i=1}^{n^{(l+1)}}W^{(l)}_{ij}\eta^{(l)}\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\varphi'(y^{(l)}_i)\partial_{x^{(l+1)}_i}L
\end{equation}
from which we can derive the variance of the gradient, based on mean field assumption, as
\begin{equation}
    \VAR{\partial_{x^{(l)}_j}L}=n^{(l+1)}(\xi^{(l)})^2(\eta^{(l)})^2\left(\frac{\gamma^{(l)}_i}{\sigma^{(l)}_i}\right)^2\VAR{W^{(l)}_{ij}}\E{(\varphi'(y^{(l)}_i))^2}\VAR{\partial_{x^{(l+1)}_i}L}
\end{equation}
Substituting~\eqref{eq:sigma}, we have
\begin{subequations}
\allowdisplaybreaks
\begin{align}
    \VAR{\partial_{x^{(l)}_j}L}&=n^{(l+1)}(\xi^{(l)})^2\cancel{(\eta^{(l)})^2}\frac{\cancel{(\gamma^{(l)}_i)^2}}{n^{(l)}\cancel{(\eta^{(l)})^2}(\rho^{(l)})^2\cancel{\VAR{W^{(l)}_{ij}}}\cancel{\E{(\varphi'(y^{(l)}_j))^2}}\cancel{(\gamma^{(l)}_j)^2}}\cancel{\VAR{W^{(l)}_{ij}}}\nonumber\\
    &\cdot \cancel{\E{(\varphi'(y^{(l)}_i))^2}}\VAR{\partial_{x^{(l+1)}_i}L}\nonumber\\
    &=\left(\frac{\xi^{(l)}}{\rho^{(l)}}\right)^2\cdot\frac{n^{(l+1)}}{n^{(l)}}\cdot\VAR{\partial_{x^{(l+1)}_i}L}
\end{align}
\end{subequations}

Ignoring spatial dependence of all statistics, we have
\begin{equation}
\boxed{
    \frac{\VAR{\partial_{x^{(l)}}L}}{\VAR{\partial_{x^{(l+1)}}L}}\approx\left(\frac{\xi^{(l)}}{\rho^{(l)}}\right)^2\cdot\frac{n^{(l+1)}}{n^{(l)}}
}
\end{equation}






==> tex_files/colored_formula.tex <==
\begin{equation}
\label{eq:software}
    \widetilde{y}=\sum_{i=1}^N\widetilde{Q}_i\widetilde{q}_i
\end{equation}

\begin{equation}
\label{eq:pim_colored}
    \widetilde{y}_{\IMC}=\textcolor{red}{\bm{\mathsf{Q}}}(\textcolor{mybrown}{\bm{\mathsf{NL}}}(\sum_{i=1}^N\widetilde{Q}_i\widetilde{q}_i);b_{\IMC})+\textcolor{myblue}{\varepsilon}
\end{equation}


\begin{equation}
\label{eq:partial_sum}
    S_i=S_{i-1}+\sum_{i=1}^N\widetilde{Q}_i\widetilde{q}_i
\end{equation}
